Translating Workflow Nets into the Partially Ordered Workflow Language

The Partially Ordered Workflow Language (POWL) has recently emerged as a process modeling notation, offering strong quality guarantees and high expressiveness. However, its adoption is hindered by the prevalence of standard notations like workflow nets (WF-nets) and BPMN in practice. This paper presents a novel algorithm for transforming safe and sound WF-net into equivalent POWL models. The algorithm recursively identifies structural patterns within the WF-net and translates them into their POWL representation. We formally prove the correctness of our approach, showing that the generated POWL model preserves the language of the input WF-net. Furthermore, we demonstrate the high scalability of our algorithm, and we show its completeness on a subclass of WF-nets that encompasses equivalent representations for all POWL models. This work bridges the gap between the theoretical advantages of POWL and the practical need for compatibility with established notations, paving the way for broader adoption of POWL in process analysis and improvement applications.

==> old-parts.tex <==
% \def\normalizestart{\ensuremath{\overleftarrow}}
% \def\normalizeend{\ensuremath{\overrightarrow}}
% \def\normalizepresetsall{\ensuremath{\overleftarrow}}
% \def\normalizepostsetsall{\ensuremath{\overrightarrow}}
% \def\normalizeall{\ensuremath{\overleftrightarrow}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Transition Reachability and Execution Order in Sound Free-Choice WF-nets}\label{sec:transition_reachability}

% In this subsection, we rigorously prove that in a sound and free-choice workflow net, if there exists a transition reachability from one transition to another, then there is a firing sequence from the initial marking to the final marking where the first transition occurs before the second.




% \begin{theorem}
% \label{thm:transition_reachability_order}
% Let $N = (P, T, l, s, f)$ be a sound and free-choice workflow net. For any two transitions $t, t' \in T$, if $t \TTR t'$, then there exists a firing sequence $\sigma$ from initial marking to the final marking such that $t$ occurs before $t'$ in $\sigma$.
% \end{theorem}

% \begin{proof}
% Assume that $t \TTR t'$ in the Petri net $N = (P, T, F, M_0, M_f)$. By the definition of the Transition Reachability Relation ($\TTR$), there exists a sequence of places and transitions connecting $t$ to $t'$. Specifically, there exist places $p_1, p_2, \ldots, p_n \in P$ and transitions $t = t_1, t_2, \ldots, t_{n+1} = t'$ such that for each $i$ ($1 \leq i \leq n$):
% \[
% t_i \in \pre{p_{i}} \quad \text{and} \quad t_{i+1} \in \post{p_i}.
% \]

% Our goal is to construct a firing sequence $\sigma$ from $M_0$ to $M_f$ where $t$ occurs before $t'$. We proceed with the following steps:

% \paragraph{(Step 1) Firing $t_1$:}
% Since $N$ is sound, every transition is \emph{live}, meaning that there exists at least one firing sequence $\sigma_0$ from $M_0$ to a marking where $t$ is enabled. After firing $t$, another marking $M_1$ is reached:
% \[
% (N, M_0) \xrightarrow{\sigma_0 \cdot \langle t \rangle} (N, M_1).
% \]


% \paragraph{(Step 2) Firing Transitions Along the Path to $t'$:}

% After firing $t=t_1$, we will show that all of the transitions $t_{2}, \ldots, t_{n+1} = t'$  can eventually be fired sequentially to reach $t_{n+1} = t'$.

% \textbf{Claim:} For each $i$ ($1 \leq i \leq n$), transition $t_{i+1}$ can eventually be enabled after firing $t_i$.


% \textbf{Proof:}
% Let us denote the marking that results after firing $t_i$ by $M_i$. Then we prove that there exist a firing sequence $\sigma_i \cdot \langle t_{i+1} \rangle \in T^* \cdot \{t_{i+1}\}$ leading from $M_i$ to a new marking $M_{i+1}$:
% \[
% (N, M_i) \xrightarrow{\sigma_i \cdot \langle t_{i+1} \rangle} (N, M_{i+1}).
% \]

% Place $p_i$ must contain a token in $M_i$ because $t_i\in \pre{p_i}$. Since $N$ is sound, the token in $p_i$ must eventually be consumed to reach the final marking. Because $N$ is free-choice, when the token in $p_i$ is consumed, any transition that consumes from $p_i$ can be chosen to fire because, by the definition of free-choice nets, all transitions in the post-set of $p_i$ must share the same pre-sets. Therefore, transition $t_{i+1}$ can be fired at some point after $t$, i.e., there must exist a firing sequence $\sigma_i \cdot \langle t_{i+1} \rangle$ from $M_i$ that ends by firing $t_{i+1}$, leading to a new marking $M_{i+1}$:
% \[
% (N, M_i) \xrightarrow{\sigma_i \cdot \langle t_{i+1} \rangle} (N, M_{i+1}).
% \]

% Therefore, we can sequentially fire transitions $t_{2}, \ldots, t_{n+1} = t'$, resulting in a marking $M_{i+1}$:
% \[
% (N, M_1) \xrightarrow{\sigma_1 \cdot \langle t_{2} \rangle \cdot \ldots \cdot \sigma_n \cdot \langle t_{n+1} \rangle} (N, M_{n+1}).
% \]

% \paragraph{(Step 3) Reaching the Final Marking:}

% Since $N$ is sound, from any reachable marking (including $M_{n+1}$), there exists a firing sequence $\sigma_{n+1}$ that leads to the final marking $M_f$:
% \[
% (N, M_{n+1}) \xrightarrow{\sigma_{n+1}} (N, M_f).
% \]

% \paragraph{Constructing the Complete Firing Sequence}

% Combining the sequences from the previous steps, we construct the firing sequence $\sigma$:
% \[
% \sigma = \sigma_0 \cdot \langle t_{1} \rangle \cdot \sigma_1 \cdot \langle t_{2} \rangle \cdot \ldots \cdot \sigma_n \cdot \langle t_{n+1} \rangle \cdot \sigma_{n+1}
% \]
% with
% \[
% (N, M_0) \xrightarrow{\sigma} (N, M_f).
% \]
% This sequence starts from $M_0$ and reaches $M_f$, with $t = t_{1}$ occurring before $t' = t_{n+1}$. This completes the proof.
% \end{proof}

% \section{Projection and Workflow Net Normalization}

% In this section, we define how to project a Petri net onto a given subset of transitions and ensure that the resulting sub-net forms a proper workflow net. We also define how to revert this transformation if needed.


% \begin{definition}[Projection Function]\label{def:projection}
% Let $N = (P, T)$ be a Petri net, and let $I \subseteq P$ and $F \subseteq P$ be sets of initial and final places, respectively. Let $T' \subseteq T$ be a subset of transitions. The \emph{projection function} 
% \[
% \xorproject(N, I, F, T') = (N_{new}, I_{new}, F_{new})
% \]
% constructs a sub-net $N_{new} = (P_{new}, T_{new})$ as follows:

% \begin{itemize}
%     \item $T_{new} = T'$.
%     \item $P_{new} = \{(T_1 \cap T', T_2 \cap T') \mid ({T_1}, {T_2}) \in P \ \wedge \ T' \cap (T_1 \cup T_2) \neq \emptyset\}$.

%     \item $I_{new} = \{p \in P_{new} \ | \ p \in I \ \vee \ \pre{p} = \emptyset\}$.
%     \item $F_{new} = \{p \in P_{new} \ | \ p \in F \ \vee \ \post{p} = \emptyset\}$.

% \end{itemize}


% \end{definition}



% \begin{theorem}[Free-Choice Preservation]\label{thm:free_choice_preservation}
% Let $N = (P, T)$ be a \emph{free-choice} Petri net, and let $I \subseteq P$, $F \subseteq P$, and $T' \subseteq T$. Then, the projected Petri net 
% \[
% \xorproject(N, I, F, T') = (N_{\mathit{new}}, I_{\mathit{new}}, F_{\mathit{new}})
% \]
% is also a \emph{free-choice} Petri net.
% \end{theorem}

% \begin{proof}

% For any two distinct transitions $t, t' \in T_{\mathit{new}}$, if they share a common input place in $N_{\mathit{new}}$ (i.e., $\pre{t} \cap \pre{t'} \neq \emptyset$), then in the original net $N$, they have the same pre-sets due to the free-choice property, i.e., $P_{pre} = \{(T_1, T_2) \in P \ | \ t \in T_2\} = \{(T_1, T_2) \in P \ | \ t' \in T_2\}$. 

% Since $P_{new}$ in $N_{\mathit{new}}$ is derived from intersecting the original places with $T'$, the equality is preserved and the presets of of $t$ and $t'$ in $N_{new}$ are equal to $\{(T_1 \cap T', T_2 \cap T') \mid ({T_1}, {T_2}) \in P_{pre}\}$. Therefore, $N_{\mathit{new}}$ satisfies the free-choice condition.
% \end{proof}





% \section{Correctness of the Choice Detection}\label{sec:correctness_choice}

% \begin{theorem}[Correctness of XOR Conversion Algorithm]
% Let $N = (P, T, \lab)$ be a sound and free-choice workflow net. Let $G = \{T_1, \ldots, T_n\}$ be the partitioning returned by Algorithm \ref{alg:choice_detection}. $G$ the partitioning of $T$ of maximal size that corresponds to an XOR structure in the language of $N$. Formally: 
% \begin{enumerate}
%     \item[\textbf{(→)}] $\lang(N) = \bigcup_{1 \leq i \leq n} \lang(N) \cap {T_i}^*$.
%     \item[\textbf{(←)}] If a subset of transitions $T' \subseteq T$ fulfills $\lang(N) \subseteq {T'}^* \cup ({T \setminus T'})^*$, then there must exists $T_1, \ldots, T_m \in G$ such that $T' = \bigcup_{1 \leq i \leq m} T_i$  
% \end{enumerate}

% \end{theorem}

% \begin{proof}

% \emph{Proof of (→):}

% Let $\sigma \in \lang(N)$ and $t_1 = \sigma(1)$. All transitions $t' \in \sigma$ within the trace $\sigma$ must be reachable from its start transition $t_1$, i.e., $t_1 \TTR t'$. Therefore, according to \autoref{alg:choice_detection}, all transitions in $\sigma$ must belong to a single group $T_i \in G$. Therefore, $\sigma \in \lang(N) \cap {T_i}^*$ for some $T_i \in G$.


% \emph{Proof of (←):}

% Assume that there exists a subset of transitions $T' \subseteq T$ such that every trace in $\lang(N)$ consists solely of transitions from $T'$ or transitions from $T \setminus T'$. Formally, $\lang(N) \subseteq {T'}^* \cup ({T \setminus T'})^*$.

% Suppose, for contradiction, that $T'$ is not a union of some groups in $G$. Then, there must exist a group $T_i \in G$ such that $T_i \cap T' \neq \emptyset$ and $T_i \setminus T' \neq \emptyset$. There must exist at least one $t_i \in T_i \cap T'$ and one $t_j \in T_i \setminus T'$ such that either $t_i \TTR t_j$ or $t_j \TTR t_i$ (otherwise, $T_i \cap T'$ and $T_i \setminus T'$ would have been discovered as separate groups by DetectXOR and not merged into $T_i$). By \autoref{thm:transition_reachability_order}, there exists $\sigma \in \lang(N)$ that contain both $t_i \in T'$ and $t_j \in T \setminus T'$. This contradicts the assumption that $\lang(N) \subseteq {T'}^* \cup ({T \setminus T'})^*$.



% \end{proof}

% \section{Correctness of the Loop Detection}\label{sec:correctness_loop}

% \begin{theorem}[Correctness of Loop Detection Algorithm] Let $N = (P, T, \lab)$ be a sound and free-choice workflow net with a unique start place $s \in P$ and a unique end place $e \in P$. The loop detection algorithm in \autoref{alg:convert_pn_to_powl} correctly identifies loop structures in $N$. Formally: The algorithm identifies a loop structure $G=\{T_{do}, T_{redo}\}$ if and only if $\lang(N) = (\lang(N) \cap (T_{do})^*) \cdot ((\lang(N) \cap (T_{redo})^*) \cdot (\lang(N) \cap (T_{do})^*))^*$.
% \end{theorem}

% \paragraph{Proof of (1):} Assume that the loop detection algorithm identifies a loop structure in $N$, i.e., it finds non-empty, disjoint subsets $T_{do}$ and $T_{redo}$ satisfying the conditions: 


% \begin{enumerate} \item $T_{do} = \PTR(s, e) \neq \emptyset$, \item $T_{redo} = \PTR(e, s) \neq \emptyset$, \item $T_{do} \cap T_{redo} = \emptyset$, \item $T = T_{do} \cup T_{redo}$. \end{enumerate}

% By the definition of $\PTR$, the set $T_{do}$ contains all transitions that are reachable from $s$ and can reach $e$ without passing through $e$ beforehand. Similarly, $T_{redo}$ contains all transitions that are reachable from $e$ and can reach $s$ without passing through $s$ beforehand.

% Since $T_{do}$ and $T_{redo}$ are disjoint and cover all transitions in $T$, we can partition the net into two subnets: \begin{itemize} \item The \emph{do-part} $N_{do}$ consisting of transitions in $T_{do}$ and places on paths from $s$ to $e$. \item The \emph{redo-part} $N_{redo}$ consisting of transitions in $T_{redo}$ and places on paths from $e$ back to $s$. \end{itemize}

% In a sound workflow net, starting from the initial marking $M_0$ (with a token in $s$), we can execute transitions in $T_{do}$ to reach a marking $M_e$ (with a token in $e$). From $M_e$, we have two options: \begin{enumerate} \item Terminate the execution if $e$ is the final place, reaching the final marking $M_f$. \item Execute transitions in $T_{redo}$ to return to a marking $M_s$ (with a token back in $s$), effectively looping back to the start. \end{enumerate}

% Because $N$ is sound and free-choice, and transitions in $T_{do}$ and $T_{redo}$ are disjoint, we can repeat this process any number of times. This means that any trace in the net starts with a sequence from the do-part, possibly followed by zero or more repetitions of sequences from the redo-part and the do-part. Therefore, the language of the net can be expressed as: $\lang(N) = (\lang(N) \cap (T_{do})^*) \cdot ((\lang(N) \cap (T_{redo})^*) \cdot (\lang(N) \cap (T_{do})^*))^*$



% \paragraph{Proof of (2):}

% Assume that there exist non-empty, disjoint subsets \( T_{do} \) and \( T_{redo} \) of \( T \), satisfying \( T = T_{do} \cup T_{redo} \), such that:

% \[
% \lang(N) = M_{do} \cup (M_{do} \cdot M_{redo} \cdot M_{do}) \cup \ldots.
% \]
% where $M_{do} \subseteq {T_{do}}^*$ and $M_{redo} \subseteq {T_{redo}}^*$ are the non-empty sets of loop-projections of $\lang(N)$ on $T_{do}$ and $T_{redo}$ respectively.

% Our goal is to show that:

% \begin{enumerate}
%     \item \( T_{do} = \PTR(s, e) \),
%     \item \( T_{redo} = \PTR(e, s) \).
% \end{enumerate}

% \paragraph{Showing that \( \PTR(s, e) \subseteq T_{do} \):}

% Let \( t \in \PTR(s, e) \). By definition, there exists a sequence of places and transitions leading from \( s \) that includes \( t \) without reaching \( e \) beforehand. Suppose, for contradiction, that \( t \in T_{redo} \). According to the language decomposition, after executing \( T_{do} \), the process can either terminate or execute \( T_{redo} \). If \( t \in T_{redo} \), it would imply that \( e \) is reached before \( t \), which contradicts the fact that \( t \) is reachable from \( s \) without passing through \( e \) first. Therefore, \( t \) must belong to \( T_{do} \), and hence:
% \[
% \PTR(s, e) \subseteq T_{do}.
% \]

% \paragraph{Showing that \( T_{do} \subseteq \PTR(s, e) \):}

% Let \( t \in T_{do} \). By the language decomposition, the set of sequence from $s$ hat do not reach $e$ (i.e., does not contain a prefix that corresponds to a valid sequence) must consist solely of transitions in \( T_{do} \). Therefore, \( t \) lies on a path from \( s \) to \( e \) without passing through \( e \) beforehand. Hence:
% \[
% T_{do} \subseteq \PTR(s, e).
% \]

% \paragraph{Combining the Inclusions for \( T_{do} \):}

% From the above two inclusions, we conclude that:
% \[
% T_{do} = \PTR(s, e).
% \]


% \paragraph{Showing that \( T_{redo} = \PTR(e, s) \):}

% \emph{First, we show that \( T_{redo} \subseteq \PTR(e, s) \).}

% Let \( t \in T_{redo} \). In the language \( \lang(N) \), after sequences from \( T_{do} \), sequences from \( T_{redo} \) can occur, allowing the process to return to \( s \) from \( e \). This means that there exists a firing sequence starting from a marking with a token at \( e \), passing through \( t \), and reaching a marking with a token at \( s \). Therefore, \( t \in \PTR(e, s) \), and thus:

% \[
% T_{redo} \subseteq \PTR(e, s).
% \]

% \emph{Next, we show that \( \PTR(e, s) \subseteq T_{redo} \).}

% Let \( t \in \PTR(e, s) \). By the definition of \( \PTR \), there exists a sequence of places and transitions leading from \( e \) back to \( s \) that includes \( t \). In the language decomposition, after reaching \( e \) via \( T_{do} \), the only transitions that can occur to return to \( s \) are from \( T_{redo} \). Therefore, \( t \in T_{redo} \), and hence:

% \[
% \PTR(e, s) \subseteq T_{redo}.
% \]

% \emph{Combining the two inclusions, we have:}

% \[
% T_{redo} = \PTR(e, s).
% \]


% \paragraph{Handling the Case Where \( s = e \):}

% If \( s = e \), the net may represent a self-loop without a distinct \emph{do-part}. In this case, the language decomposition simplifies to:

% \[
% \lang(N) = \left( (\lang(N) \cap T_{redo}^*) \cdot (\lang(N) \cap T_{do}^*) \right)^*.
% \]

% The loop detection algorithm handles this scenario by applying the \texttt{selfloop} preprocessing function (see \autoref{def:self_loop_preprocessing}). This function introduces a silent transition \( t_{do} \) and creates distinct places \( source \) and \( sink \), effectively creating an explicit do-part.

% After preprocessing:

% \begin{itemize}
%     \item \( T_{do} = \{ t_{do} \} \) (the silent transition modeling the do-part),
%     \item \( T_{redo} = T \setminus \{ t_{do} \} \) (the original transitions modeling the redo-part).
% \end{itemize}

% Applying the same reasoning as before, we conclude that \( T_{do} = \PTR(source, sink) \) and \( T_{redo} = \PTR(sink, source) \), confirming that the algorithm correctly identifies the loop structure.

% \paragraph{Overall Conclusion:}

% The loop detection algorithm identifies loop structures in \( N \) if and only if the language \( \lang(N) \) can be decomposed as:

% \[
% \lang(N) = (\lang(N) \cap T_{do}^*) \cdot \left( (\lang(N) \cap T_{redo}^*) \cdot (\lang(N) \cap T_{do}^*) \right)^*,
% \]

% with \( T_{do} = \PTR(s, e) \) and \( T_{redo} = \PTR(e, s) \). This completes the proof of the second direction.


% \subsection{Reachability Graph}\label{sec:reachability_graph}

% The \emph{reachability graph} is a fundamental concept in the analysis of Petri nets, capturing all possible states (markings) that the net can attain from an initial marking through the firing of transitions. It provides a comprehensive view of the dynamic behavior of the net, facilitating the verification of properties such as liveness, boundedness, and soundness.

% \subsubsection{Markings}

% A \emph{marking} is a multi-set of places indicating the number of tokens present in each place at a given state of the Petri net. Formally, for a Petri net $N = (P, T, \lab)$, a marking $M \in \bag(P)$ assigns a non-negative integer number of tokens to each place in $P$.

% \begin{definition}[Marking]
%     Let $N = (P, T)$ be a Petri net. A \emph{marking} is a function $M \colon P \to \Nat$ where $M(p)$ denotes the number of tokens in place $p \in P$. The set of all possible markings of $N$ is denoted by $\MarkingSet(N) = \bag(P)$.
% \end{definition}

% \subsubsection{Transition Firing}

% Transitions in a Petri net can fire when they are \emph{enabled}, meaning that each of their preceding places has at least one token. Firing a transition consumes one token from each of its preceding places and produces one token in each of its succeeding places.

% \begin{definition}[Transition Firing]
%     Let $N = (P, T)$ be a Petri net and $M \in \MarkingSet(N)$ be a marking. A transition $t \in T$ is \emph{enabled} in $M$ if for every place $p$ such that $p$ is a predecessor of $t$ (i.e., $p$ has an outgoing arc to $t$), $M(p) \geq 1$.

%     When an enabled transition $t$ fires, it results in a new marking $M' \in \MarkingSet(N)$ defined by:
%     \[
%     M'(p) =
%     \begin{cases}
%         M(p) - 1 & \text{if } p \text{ is a predecessor of } t, \\
%         M(p) + 1 & \text{if } p \text{ is a successor of } t, \\
%         M(p) & \text{otherwise}.
%     \end{cases}
%     \]
%     We denote this firing as $(N, M) \xrightarrow{t} (N, M')$.
% \end{definition}

% \subsubsection{Reachability Graph}

% The reachability graph provides a complete representation of all possible markings reachable from an initial marking through sequences of transition firings.

% \begin{definition}[Reachability Graph]
%     Let $N = (P, T)$ be a Petri net and $M_0 \in \MarkingSet(N)$ be the initial marking. The \emph{reachability graph} of $N$ from $M_0$, denoted by $\RG(N, M_0)$, is a directed graph defined as follows:
%     \begin{itemize}
%         \item \textbf{Nodes}: Each node represents a unique marking $M \in \MarkingSet(N)$ that is reachable from $M_0$ via a sequence of transition firings.
%         \item \textbf{Edges}: There is a directed edge labeled $t \in T$ from node $M$ to node $M'$ if and only if $(N, M) \xrightarrow{t} (N, M')$, i.e., transition $t$ is enabled in marking $M$ and its firing results in marking $M'$.
%     \end{itemize}
%     Formally,
%     \[
%     \RG(N, M_0) = (V, E)
%     \]
%     where
%     \[
%     V = \{ M \in \MarkingSet(N) \mid \exists \sigma \in T^* \ \text{such that} \ (N, M_0) \xrightarrow{\sigma} (N, M) \},
%     \]
%     and
%     \[
%     E = \{ (M, M', t) \mid M, M' \in V \ \wedge \ (N, M) \xrightarrow{t} (N, M') \}.
%     \]
% \end{definition}


% \begin{algorithm}[H]
% \caption{Choice Detection in Petri Nets}\label{alg:choice_detection}
% \DontPrintSemicolon
% \KwIn{Petri net $N = (P, T)$}
% \KwOut{A partitioning $G \in \allPart(T)$ representing choice branches.}

% \SetKwFunction{FMain}{DetectXOR}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FMain{$N$}}{
%     $G \leftarrow \{\{t\} \ | \ t \in T\}$  
    
%     \For{$(t_1, t_2) \in T \times T$ where $t_1 \neq t_2$}{
%         \If{$t_1 \TTR t_2$ or $t_2 \TTR t_1$}{
%             $G \leftarrow G \setminus \{G_{t_1}, G_{t_2}\} \cup \{G_{t_1} \cup G_{t_2}\}$  
%         }
%     }
%     \KwRet{$G$}
% }
% \end{algorithm}

% We initially assign each transition to a separate subset and then merge subsets only when they share transitions with overlapping transition reachabilities. If $DetectXOR(N)$ consists of multiple subsets, then a choice structure is detected over the identified subsets; otherwise, no choice is detected. 


% \begin{definition}[System Net Projection]\label{def:projection}
% Let $N = (P, T, \{source\}, \{sink\})$ be a safe system net with unique source and sink places. Let $T' \subseteq T$ be a subset of transitions. The \emph{projection} of $N$ on $T'$ is defined as: 
% \[
% \xorproject(N, T') = (P', T', \{source'\}, \{sink'\})
% \]
% where

% \begin{itemize}
%     \item $P' = \{(T_1 \cap T', T_2 \cap T') \mid ({T_1}, {T_2}) \in P \ \wedge \ T' \cap (T_1 \cup T_2) \neq \emptyset\}$.

%     \item $source' = (\emptyset, \post{source} \cap T')$.

%     \item $sink' = (\pre{sink} \cap T', \emptyset)$.

% \end{itemize}
% \end{definition}

% \begin{theorem}[Projection Preserves Soundness]
% \label{thm:projection_soundness}
% Let $SN = (N, I, F)$ be a safe and sound system net, where $N = (P, T)$ is the underlying Petri net, and $I, F \subseteq P$ are the sets of initial and final places, respectively. Let $T' \subseteq T$ be a subset of transitions. Then, $\xorproject(N, T')$ is safe and sound.
% \end{theorem}

% \subsection{Petri Net Normalization}\label{sec:reachability_relations}

% \begin{definition}[Normalized Petri Net]\label{def:projection}
% Let $SN = (N, I, F)$ with $ N = (P, T)$ be a safe system net. We construct 
% \[
% \normalizepn(N, I, F) = (N_{new}, [i_{new}], [f_{new}])
% \]
% with $N_{new} = (P_{new}, T_{new})$ as follows:

% \begin{itemize}
%     \item $T_{new} = T \cup \{t_{start}, t_{end}\}$ where $t_{start}, t_{end} \notin T$ with $t_{start} \neq t_{end}$ and $\lab(t_{start}) = \lab(t_{end}) = \tau$.
%     \item $i_{new} = (\emptyset, {t_{start}})$
%     \item $f_{new} = ({t_{end}}, \emptyset)$
%     \item $P_{new} = \{I_{new}, F_{new}\} \cup \{(f_1(p), f_2(p)) \mid p \in P \}$ where 
%     \[
%     f_1(p) =
%     \begin{cases}
%         \pre{p} \cup \{t_{start}\} & \text{if } p \in I, \\
%         \pre{p} & \text{otherwise}.
%     \end{cases}
%     \]
%     and 
%     \[
%     f_2(p) =
%     \begin{cases}
%         \post{p} \cup \{t_{end}\} & \text{if } p \in F, \\
%         \post{p} & \text{otherwise}.
%     \end{cases}
%     \]

% \end{itemize}
% \end{definition}

% \begin{definition}[System Net Soundness]\label{def:projection}
% Let $SN = (N, I, F)$ be a safe system net. We call $(N, I, F)$ sound if $\normalizepn(N, I, F)$ is a sound WF-net.

% \end{definition}

% \begin{definition}[Free-Choice Petri Net]
% \label{def:free_choice}
% A Petri net $N = (P, T)$ is called \emph{free-choice} if for any two transitions $t_1, t_2 \in T$, whenever they share a common input place, their pre-sets are identical. Formally, $N$ is free-choice if for all $t_1, t_2 \in T$:
% \[
% (\pre{t_1} = \pre{t_2}) \quad \text{ or } \quad (\pre{t_1} \cap \pre{t_2} = \emptyset).
% \]
% \end{definition}

% \begin{definition}[WF-Net Component]\label{def:comp}
% Let $N = (P, T, F)$ be a WF-Net and $T' \subseteq T$.  $\xorproject(N, T') = (P', T', F')$ is a component of $N$ if there exist $p_{source}, p_{sink} \in P'$ such that:
% \begin{itemize}
%     \item $\bullet x \subseteq T' \cup (P' \setminus \{p_{sink}\})$ for all $x \in T' \cup (P' \setminus \{p_{source}\})$.
%     \item $x \bullet \subseteq T' \cup (P' \setminus \{p_{source}\})$ for all $x \in T' \cup (P' \setminus \{p_{sink}\})$.
% \end{itemize}
% \end{definition}

% \begin{theorem}[Component Guarantees]\label{thm:comp}
% Let $N = (P, T, F)$ be a WF-Net and $N'$ be a component of $N$. Then, the following holds:
% \begin{itemize}
%     \item $N'$ is a WF-net.
%     \item If $N$ is safe and sound, then $N'$ is safe and sound.
% \end{itemize}
% \end{theorem}

% \begin{proof}
%     See \cite[Theorem 2]{van2005translating}.
% \end{proof}

% \begin{enumerate}

    % \item We prove $N_{source} \in P_i$ and $N_{sink} \in P_i$:\\
    % Consider any $t \in T_i$. Since $N$ is a sound WF-net, there is a path from $N_{source}$ to $t$ in $N$. Let $t'$ be the first transition on this path. Then $(N_{source}, t') \in F$. If $t' \in T_i$, then $N_{source} \in P_i$ by definition of the projection. If $t' \notin T_i$, then by the XOR-pattern definition, no subsequent transition on this path can be in $T_i$, contradicting the reachability of $t$ from $N_{source}$. Therefore, there must hold that $N_{source} \in P_i$.  The proof of the existence of $p_{sink}$ in $P_i$ is analogous. 

    % \item We prove that $\pre{N_{source}} = \emptyset = \post{N_{sink}}$ in $N_i$:\\ 
    % this is guaranteed by the construction of the projection since $\pre{N_{source}} = \emptyset = \post{N_{sink}}$ in $N$ and no additional flow relations are adding in the projection.

    % \item We prove that no $p \in  P_i\setminus\{N_{source}\}$ exists such that $\pre{p} = \emptyset$ in $N_i$:\\ Assume such a place exists. Since the place is included in the projected net, this implies that a transition $t \in T_i$ exists such that $(p, t) \in F$, Since $N$ is a WF-net, we conclude that $\pre{N_{source}} \neq \emptyset$, i.e., another transition $t' \in T_i$ exists such that $(t', p)\in F$. Therefore, we conclude that $t' \TTR t$. By the XOR Partitioning definition, we conclude that $t' \in T_i$ and therefore $t' \in \pre{p}$ in $N_i$, contradicting our assumption.
    
    % \item The proof that no $p \in  P_i\setminus\{N_{sink}\}$ exists such that $\post{p} = \emptyset$ in $N_i$ is analogous.\\
    
% \end{enumerate}

% \textbf{(i) }


% \textbf{(ii) We prove the two conditions of Definition \ref{def:comp}.}

% We start with the first condition [$\pre{x} \subseteq T_i \cup (P_i \setminus \{N_{sink}\})$ for any $x \in T_i \cup (P_i \setminus \{N_{source}\})$]:

% \begin{itemize}
%     \item Case 1 ($x \in T_i$): Let \(p \in \bullet x\) in \(N\).  This means \((p, x) \in F\). Since \(x \in T_i\), by the definition of projection, \(p \in P_i\). Now, assume \(p = N_{sink}\). This would imply \((N_{sink}, x) \in F\), contradicting $\post{N_{sink}} = \emptyset$ (c.f. \autoref{def:wfn}). Therefore, we conclude that $p \in (P_i \setminus \{N_{sink}\})$.
    
%     \item Case 2 (\(x \in P_i \setminus \{N_{source}\}\)): 

%     \begin{itemize}
%         \item Case 2.1 ($x = N_{sink}$):
%         \item Case 2.2 ($x \in P_i \setminus \{N_{source}, N_{sink}\}$): there must exist at least one \(t \in (\pre{x} \cap T_i) \cup (\post{x} \cap T_i)\) since $x$ is included in the projected net $N_i$. Without loss of generality, assume \(t \in \pre{x} \cap T_i \). Now, for any \(t' \in \post{x}\) in \(N\), we have \(t \TTR t'\). By the XOR-pattern definition, we must have \(t' \in T_i\). Similarly, we have \(t'' \TTR t'\) and, therefore \(t'' \in T_i\), for any $t'' \in \pre{t'}$. We conclude that $\pre{x} \subseteq T_i$.

%     \end{itemize}

    
% \end{itemize}
% Therefore, the condition holds for all $x \in T_i \cup (P_i \setminus \{p_{source}\})$.  

% \textbf{Second condition [$\post{x} \subseteq T_i \cup (P_i \setminus \{N_{source}\})$ for any $x \in T_i \cup (P_i \setminus \{N_{sink}\})$]:} The proof is analogous to the first condition.


% Thus, $N_i$ is a component of $N$. Since $N$ is a safe and sound WF-net, by Theorem \ref{thm:comp}, $N_i$ is a safe and sound WF-net.

% \begin{definition}[XOR-Pattern]
% Let $N = (P, T, F)$ be a safe and sound WF-net. Let $G = \{T_1, \ldots, T_n\} \in \AllPart(T)$ be a partitioning of transitions of size $n > 1$. The tuple $(N, G)$ is called an XOR Pattern if and only if for all $(t, t') \in T \times T$:
% \[
% \text{if } t \TTR t' \text{, then } G_t = {G_{t'}}.
% \]
%  \end{definition}

% \begin{definition}[XOR Projection]\label{def:projection_xor}
% Let $(N, G)$ be an XOR Pattern with $N = (P, T, F)$ and $T' \in G$ be a subset of transitions. The XOR projection of $N$ on $T'$ is defined as $\xorproject(N, T') = (P', T', F')$ where $P' = P\project{T'}$ and $F' = F\project{P', T'}$.

% % \[
% % P' = \{ p \in P \ | \ \pre{p} \subseteq T' \ \wedge \ \post{p} \subseteq T' \} \cup \{N_{source}, N_{sink}\}
% % \]
% % and
% % \[
% % F' = F \cap ((P' \times T') \cup (T' \times P')).
% % \]

% Consider any $t \in T_i$. Since $N$ is a sound WF-net, there is a path that starts from $N_{source}$, goes through $t$, and ends in in $N_{sink}$. Then the first and last transitions in this path, say $t_{start}$ and $t_{end}$, must be both in $T_i$ since $t_{start} \TTR t$ and $t \TTR t_{end}$. These two transitions must be connected to $N_{source}$ and $N_{sink}$, respectively. By construction of $N_i$, we know that $N_{source} \in P_i$ and $N_{sink} \in P_i$ are the unique source and sink places in $N_i$, respectively. Now we need to show that all transitions in the projected net remain connected. Assume for contradiction that there exists a place $p \in P \setminus \{N_{source}, N_{sink}\}$ connecting transitions from both $T_i$ and $T \setminus T_i$ and therefore not included in $P'$. Without loss of generality, we assume there exist $t \in T_i$ and $t' \in (T \setminus T_i)$ such that $(t, p) \in F$ and $(p, t') \in F$. Then $t \TTR t'$, and by the XOR-Pattern definition, the two transitions must be placed within the same subset, which contradict our assumption that $t \in T_i$ and $t' \in (T \setminus T_i)$. Therefore, the projected net must remain connected.

% The proof that $N'$ is a WF-net with the unique source and sink places $N_{source}$ and $N_{sink}$, respectively, is analogous to (i). $N$ can be reconstructed from $N'$ as described in \cite[Theorem 3.4]{compTheorem} by replacing $t^{\texttt{+}}$ by $N_i$ if $P = P_i \cup P'$, Assume for contradiction that there exists a place $p\in P \setminus (P_i \cup P')$. Then this place must be connecting transitions from both $T_i$ and $T \setminus T_i$, which is not possible as we showed in the proof of (i). Therefore, we conclude that $P = P_i \cup P'$, and by \cite[Theorem 3.4]{compTheorem}, $N_i$ is safe and sound. 

% \item $\{(N_{source}, t_{source})\} = \{(p, t) \in F \ | \ p = N_{source} \text{ or } t = t_{source} \}$,
    % \item $\{(t_{sink}, N_{sink})\} = \{(t, p) \in F \ | \ t = t_{sink} \text{ or } p = N_{sink} \}$,

    % \[
% P' = \{ p \in P \ | \ \pre{p} \subseteq T' \ \wedge \ \post{p} \subseteq T' \} \cup \{N_{source}, N_{sink}\}
% \]

% By construction, $N_{source}$ and $N_{sink}$ are the unique source and sink places in $N_{do}$, respectively. Now we need to show that all transitions and places in $N_{do}$ are on a path from $N_{source}$ to $N_{sink}$. Consider any $t \in T_{do}$. By definition of a Loop-Pattern and $T_{do}$, there exists a path from $p_{do}$ to $p_{redo}$ in $N$ that contains solely transitions from $T_{do}$, including t. The loop projection replaces all flow connections $(p_{do}, t)$ by $(N_{source}, t)$ and all flow connections $(t, p_{redo})$ by $(t, N_{sink})$. Therefore, we conclude that all transitions and places in $T_{do}$ are on a path from $N_{source}$ to $N_{sink}$ in $N_{do}$ if no place $p \in P \setminus \{p_{do}, p_{redo}\}$ connecting transitions from both $T_{do}$ and $T_{redo}$ exists (i.e., $p$ is not included in $P_{do}$). Assume for contradiction that such a place exists. Without loss of generality, assume that there exist transitions $t \in T_{do}$ and $t' \in T_{redo}$ where $(t,p) \in F$ and $(p,t') \in F$. This means that in the original net $N$, there is a path starting from $p_{do}$ to $t$, without passing through $p_{redo}$ in-between. From $t$, the path can continue through $p$ to reach $t'$. From $t'$, we know that we can eventually reach $p_{redo}$ (either $p_{redo}$ lies on path from $t'$ to $p_{do}$ or we reach $p_{do}$ first and then take any path from $p_{do}$ to $p_{redo}$). Combining all of these sequences ($p_{do} \rightarrow \ldots \rightarrow t \rightarrow p \rightarrow t' \rightarrow ... \rightarrow p_{redo})$ implies that $t' \in T_{do}$. This contradicts our initial assumption that $t' \in T_{redo}$ and the fact that $T_{do}$ and $T_{redo}$ are disjoint subsets. Therefore, no such place $p$ can exist, and all transitions and places in $N_{do}$ are on a path from $N_{source}$ to $N_{sink}$. This shows that $N_{do}$ is a WF-net.

    % \item $P' = \{ p \in P \ | \ \pre{p} \subseteq T' \ \wedge \ \post{p} \subseteq T' \} \cup \{p_{do}, p_{redo} \}$.
    % \item $F' = (F \cap ((T'\times P') \cup (P' \times T'))) \cup \{(N_{do}, t^{\texttt{+}}), (t^{\texttt{+}}, N_{redo})\}$.

% \begin{definition}[Partial Order Pattern]\label{def:po_pattern}
% Let $N = (P, T, F)$ be a safe and sound WF-net. Let $G = \{T_1, \ldots, T_n\} \in \AllPart(T)$ be a partitioning of transitions of size $n > 1$. The tuple $(N, G)$ is called a partial order pattern if and only if the following conditions hold: 
% \begin{itemize}
%     \item For all $t, t' \in T$ and $p \in P$:
%     \[
%         \text{if } t, t' \in \{t \in T \ | \ \exists_{t_1, t_2 \in \post{p}} \ t_1 \TTR t \wedge t_2 \notTTR t \}\text{, then } G_{t} = G_{t'}.
%     \]
    % \item A partial order $\po$ over  $\{1, \ldots, n\}$ exists such that for all $i, j \in \{1, \ldots, n\}$, $P' = \{p \in P \ | \ (T_i \times T_j) \cap (\pre{p} \times \post{p}) \neq \emptyset\}$:
    % \[
    %     i \reduction{\po} j \Leftrightarrow P' \neq \emptyset
    % \]
    % and
    % \[
    %     (\forall_{p, p' \in P'}\ \pre{p}\cap T_i = \pre{p'}\cap T_i) \ \vee \  (\forall_{p, p' \in P'}\ \post{p}\cap T_j = \post{p'}\cap T_j).
    % \]
    % \item A partial order $\po$ over  $\{1, \ldots, n\}$ exists such that for all $i, j \in \{1, \ldots, n\}$; $t_i \in T_i$; $t_j \in T_j$:
    % \[
    %     i \po j \Leftrightarrow t_i \TTR t_j.
    % \]


%     \begin{definition}[Preprocessing by Merging All Places with Identical Pre-sets or Post-sets]\label{def:preprocessing_all}
% Let $N = (P, T, F)$ be a Petri net. We define the preprocessing function to merge all places with identical pre-sets and all places with identical post-sets as:
% \[
% \normalizeall(N) = N_2 \text{ where } N_1 = \normalizepostsetsall(\normalizepresetsall(N))
% \]
% where
% \[
% \normalizepresetsall(N) = (P', T', F')
% \]
% is defined as follows:

% Let $G = \{S_1, S_2, ..., S_n\}$ be the set of all maximal subsets of $P$ such that for each $S_i \in G$, all places in $S_i$ have identical pre-sets (i.e., $\forall p_1, p_2 \in S_i: \pre{p_1} = \pre{p_2}$), and for any $p \notin S_i$, $\pre{p} \neq \pre{p'}$ for all $p' \in S_i$.

% \begin{itemize}
%     \item $P' = P \cup \{p_S \ | \ S \in G \}$ where each $p_S \notin P$ is a new place.
%     \item $T' = T \cup \{t_S \ | \ S \in G \}$ where each $t_S \notin T$ is a new silent transition with $\lab(t_S) = \tau$.
%     \item $F_{remove} = \{(t, p) \in F \ | \ p \in S, S \in G\} \cup \{(p, t) \in F \ | \ p \in S, S \in G, \forall_{p \in S}\ (p, t) \in F \}$ 
%     \item $F' = (F \setminus F_{remove}) \\
%     \cup \{(t, p_S) \ | \ S \in G, p \in S, (t, p) \in F \} \\
%     \cup \{(p_S, t_S) \ | \ S \in G \} \\
%     \cup \{(t_S, p) \ | \ S \in G, p \in S\} \\
%     \cup \{(p_S, t) \ | \ S \in G \ \wedge \ \forall_{p \in S}\ (p, t) \in F \}$.
%     % \cup \{(p, t) \ | \  (p, t) \in F \ \wedge \ \exists_{S \in G} \ (p \in S \ \wedge \ \exists_{p' \in S}\ (p', t) \notin F) \}$.
% \end{itemize}

% And
% \[
% \normalizepostsetsall(N) = (P', T', F')
% \]
% is defined analogously:

% Let $\mathcal{E} = \{E_1, E_2, ..., E_m\}$ be the set of all maximal subsets of $P$ such that for each $E_j \in \mathcal{E}$, all places in $E_j$ have identical post-sets (i.e., $\forall p_1, p_2 \in E_j: \post{p_1} = \post{p_2}$), and for any $p \notin E_j$, $\post{p} \neq \post{p'}$ for all $p' \in E_j$.

% \begin{itemize}
%     \item $P' = (P \setminus \bigcup_{E \in \mathcal{E}} E) \cup \{p_E \ | \ E \in \mathcal{E} \}$ where each $p_E \notin P$ is a new place.
%     \item $T' = T \cup \{t_E \ | \ E \in \mathcal{E} \}$ where each $t_E \notin T$ is a new silent transition with $\lab(t_E) = \tau$.
%     \item $F' = (F \setminus \{(p, t) \ | \ p \in E, E \in \mathcal{E}, t \in \post{p}\}) \\
%     \cup \{(p_E, t_E) \ | \ E \in \mathcal{E} \} \\
%     \cup \{(t, t_E) \ | \ E \in \mathcal{E}, t \in \bigcup_{p \in E} \pre{p} \} \\
%     \cup \{(t_E, t) \ | \ E \in \mathcal{E}, t \in \post{p}, p \in E \}$.
% \end{itemize}

% \end{definition}

% \begin{lemma}[Properties of \(\normalizeall\)]\label{thm:preprocessing_all_properties}
% Let \(N = (P, T, F)\) be a safe and sound WF-net. Then \(N' = \normalizeall(N)\) is a safe and sound WF-net with \(\lang(N') = \lang(N)\).
% \end{lemma}

% \begin{proof}
% The proof is a straightforward extension of the proof for Lemma \ref{thm:preprocessing_properties}.

% 1. **\(N'\)  is a WF-net:**  The  `\normalizeall`  function performs the  `\normalizepresetsall`  and `\normalizepostsetsall` transformations sequentially. Each of these transformations preserves the WF-net properties (unique source and sink, connectivity) as argued in the proof of Lemma  \ref{thm:preprocessing_properties}. Since the composition of WF-net preserving transformations is also WF-net preserving,  `\normalizeall`  results in a WF-net.

% 2. **Safeness and Soundness:**  `\normalizepresetsall` and `\normalizepostsetsall` are generalizations of  `\normalizepresets`  and  `\normalizepostsets`, respectively. They perform the same merging operations but on multiple sets of places simultaneously. The arguments for safeness and soundness in Lemma \ref{thm:preprocessing_properties} still hold for each individual merge operation. Since the merge operations do not interfere with each other (they operate on disjoint sets of places), the overall transformation preserves safeness and soundness.

% 3. **Language Preservation:** The argument for language preservation is the same as in Lemma \ref{thm:preprocessing_properties}. Each silent transition added during the  `\normalizepresetsall`  or `\normalizepostsetsall`  step does not affect the observable behavior. There is a one-to-one mapping between firing sequences in  `N`  and  `N'`  that preserves the non-silent activity sequences.

% Therefore,  `N'`  is a safe and sound WF-net with  `\lang(N') = \lang(N)`.
% \end{proof}


% \begin{definition}[Normalization of Start Places]
% Let $N = (T, P, F)$ be a Petri net and $S\subseteq P$ be a subset of start places. We define  
% \[
% \normalizestart{(N, S)} = 
% \begin{cases}
%     (T, P, F) & \text{if } |S| = 1 \ \wedge \ \forall_{p \in S}\ \pre{p} = \emptyset, \\
%     (T', P', F') & \text{otherwise}.
% \end{cases}
% \]
% with $(T', P', F')$ constructed as follows:

% \begin{itemize}
%     \item $T' = T \cup \{t_{source}\}$ where $t_{source} \notin T$ is a fresh transition with $\lab(t_{start}) = \tau$,
%     \item $P' = P \cup \{p_{source}\}$ where $p_{source} \notin P$ is a fresh place,
%     \item $F' = F \cup \{(p_{source}, t_{source})\} \cup \{(t_{source}, p) \ | \ p \in S\}$.

% \end{itemize}
% \end{definition}

% \begin{definition}[Normalization of End Places]
% Let $N = (T, P, F)$ be a Petri net and $E\subseteq P$ be a subset of end places. We define 
% \[
% \normalizeend{(N, E)} = 
% \begin{cases}
%     (T, P, F) & \text{if } |E| = 1 \ \wedge \ \forall_{p \in E}\ \post{p} = \emptyset, \\
%     (T', P', F') & \text{otherwise}.
% \end{cases}
% \]
% with $(T', P', F')$ constructed as follows:

% \begin{itemize}
%     \item $T' = T \cup \{t_{sink}\}$ where $t_{sink} \notin T$ is a fresh transition with $\lab(t_{start}) = \tau$,
%     \item $P' = P \cup \{p_{sink}\}$ where $p_{sink} \notin P$ is a fresh place,
%     \item $F' = F \cup \{(t_{sink}, p_{sink})\} \cup \{(p, t_{sink}) \ | \ p \in E\}$.

% \end{itemize}
% \end{definition}

% Let $N$ be a Petri net and $S\subseteq P$ be a subset of start places and $E\subseteq P$ be a subset of end places. Then we define:
% \[
% \normalize{(N, S , E)} = \normalizeend{(\normalizestart{(N, S)}, E)}.
% \]

% \begin{definition}[Partial Order Projection]\label{def:projection_po}
% Let $(N, G, \po)$ be a partial order pattern with $N = (P, T, F)$. Let $T' \in G$ be a subset of transitions.  The partial order projection of $N$ on $T'$ is $\poproject(N, T) = \normalize{(N', \Pre{T'}, \Post{T'})}$ where $N' = (P', T', F')$ with $P' = P\project{T'}$ and $F' = F\project{P', T'}$.
% \end{definition}

    % \item $P' = \{ p \in P \ | \ \pre{p} \subseteq T' \ \wedge \ \post{p} \subseteq T' \} \cup \{N_{source}, N_{sink}\}$.
    % \item $F' = (F \cap ((T'\times P') \cup (P' \times T'))) \cup \{(N_{source}, t^{\texttt{+}}),  (t^{\texttt{+}}, N_{sink})\}$.

    % \item $i \reduction\po j \Leftrightarrow \Post{T_i} = \Pre{T_j},$
        % \item $i \reduction\notpo j \Leftrightarrow \Post{T_i} \cap \Pre{T_j} = \emptyset,$
        % \item $|\Pre{T_i}| = |\Post{T_i}| = 1,$
        % \item $i \reduction\po j \Leftrightarrow \Post{T_i} = \Pre{T_j},$
        % \item $i \reduction\notpo j \Leftrightarrow \Post{T_i} \cap \Pre{T_j} = \emptyset.$

           % \item $i \reduction\po j \Leftrightarrow \Post{T_i} = \Pre{T_j},$
        % \item $i \reduction\notpo j \Leftrightarrow \Post{T_i} \cap \Pre{T_j} = \emptyset,$
        % \item $|\Pre{T_i}| = |\Post{T_i}| = 1,$
        % \item $i \reduction\po j \Leftrightarrow \Post{T_i} = \Pre{T_j},$
        % \item $i \reduction\notpo j \Leftrightarrow \Post{T_i} \cap \Pre{T_j} = \emptyset.$
    % \item For $P' = \Post{T_i} \cap \Pre{T_j}$:\\
    %     $(\forall_{p, p' \in P'}\ \pre{p}\cap T_i = \pre{p'}\cap T_i) \ \vee \  (\forall_{p, p' \in P'}\ \post{p}\cap T_j = \post{p'}\cap T_j)$.
    % \[
    %     i \reduction\po j \Leftrightarrow \Post{T_i} \cap \Pre{T_j} \neq \emptyset.
    % \]





The first and third conditions in the partial order pattern definition ensure that the identified "blocks" of behavior really form cleanly separable, partial-order-like components. They serve as structural "guards" that prevent pathological cases and solidify the correctness of the projection and normalization steps.

Condition 1 (Branching uniformity condition):
This condition states that if a certain place $p$ in the net leads to transitions some of which are reachable after $p$ and some are not, then all such transitions must fall into the same partition subset. Intuitively, it ensures that we do not have a single branching point $p$ that sends control flows into multiple distinct subsets $T_i, T_j$ in an unstructured manner. Without this condition, we might end up with complicated interleavings or partial overlaps between subsets, making it unclear whether each $T_i$ can be treated as a cleanly separated “block” of behavior. By enforcing that all such transitions belong to a single block, the structure of the process is more aligned with a partial order decomposition, and no unintended "cross-talk" occurs.

Condition 3 (Homogeneity of interface places):
This condition ensures that the sets of places connecting one block to another are homogeneous in terms of their incoming or outgoing transitions. Concretely, it states that at the "interfaces" between $T_i$ and $T_j$, either all interface places have the same pre-transitions from $T_i$ or the same post-transitions into $T_j$. This avoids irregular merges or splits where different places connecting the same two blocks behave differently. Such irregularities could introduce ambiguous reachability patterns or complicate the normalization by making it unclear how to form a single start or end interface for the projected net $N_i$. By enforcing this homogeneous structure, every block's interface behaves uniformly, ensuring that normalization yields a well-structured WF-net.

% \subsubsection{Identifying Basic Loops}
% In the context of identifying loops within a workflow net, we assume that the net has been preprocessed to ensure a unique start place $source$ and a unique end place $sink$. Given this assumption, we define two disjoint subsets of transitions: the \emph{redo subnet transitions}, which are the transitions reachable from the end place eventually leading back to the start place ($T_{redo} = \PTR(sink, source)$), and the \emph{do sub-net transitions}, which are the transitions reachable from the start place up to the end place ($T_{do} = \PTR(source, sink)$). If both subsets are non-empty ($T_{redo} \neq \emptyset \neq T_{do}$ ) and form a partitioning of the transitions in the net ($T = T_{redo} \cup T_{do}$ and  $T_{redo} \cap T_{do} = \emptyset$ ), we identify a loop structure. Otherwise, no loop structure is detected.

% \subsubsection{Identifying Self-Loops with Missing Do-Part}
% In some cases, a Petri net may include self-loops where the start place and end place are the same, resulting in a situation where there is no distinct \emph{do-part}. Such loops can be interpreted as cases where all activities within the loop belong to the redo-part, which can be skipped or repeated. To enable proper identification of these loops during preprocessing, we handle this special case by restructuring the Petri net.

% \begin{definition}[Self-Loop Preprocessing]\label{def:self_loop_preprocessing}
% Let $N = (P, T)$ be a Petri net with a unique start and end place $p \in P$. $\selfloop$ is a function that preprocesses $N$ to enable loop detection, i.e., $\selfloop(N, p) = (N', source, sink)$ with $N' = (P', T')$ where:
% \begin{itemize}
%     \item $
%     T' = T \cup \{t_{do}\}, t_{do} \notin T$ with $
%     \lab(t_{do}) = \tau$.
    
%     \item 
%     $
%     source = (\{t_{do}\}, \post{p}).
%     $
%     \item 
%     $
%     sink = (\pre{p}, \{t_{do}\}).
%     $
%     \item 
%     $
%     P' = P \setminus \{p\} \cup \{source, sink\}.
%     $
% \end{itemize}

% \end{definition}


% If the start and end place $p$ are the same, it is treated as a self-loop. The preprocessing function $\selfloop$ adds a silent transition $t_{do}$ and replaces $p$ with two places, $source$ and $sink$, to distinguish the do-part and redo-part. The resulting net $N'$ has $source$ as the new start place and $sink$ as the new end place. This transformation allows us to handle a self-loop as a regular loop structure where:
% \begin{itemize}
%     \item $T_{do} = \{t_{do}\}$ represents the silent transition modeling the do-part.
%     \item $T_{redo} = T' \setminus \{t_{do}\} = T$ represents the original transitions modeling the redo part of the loop.
% \end{itemize}



% \begin{definition}[Pre-Processing]\label{def:preprocessing}
% Let $N = (P, T, F)$ be a WF-net. The pre-processing function $\preprocess(N)$ simplifies the structure of the WF-net by merging places based on shared pre-sets and post-sets. The pre-processing step involves the following transformations:

% \begin{enumerate}
%     \item \textbf{Identical Pre- and Post-Sets:} If a set of places $P' \subseteq P$ shares the exact same pre-set and post-set (i.e., $\forall p_1, p_2 \in P': \pre{p_1} = \pre{p_2} \wedge \post{p_1} = \post{p_2}$), then all places in $P'$ are merged into a single place, and all incoming and outgoing arcs from/to $P'$ are redirected to this place. This transformation is illustrated in \autoref{fig:preprocessing:a}.

%     \item \textbf{Identical Pre-Sets and Different Post-Sets:} Let $P' \subseteq P$ a set of places of maximum size such that the places share the exact same pre-set but have different post-sets (i.e., $\forall_{p_1, p_2 \in P'} \ \pre{p_1} = \pre{p_2} \ \wedge \ \exists_{p_1, p_2 \in P'}\ \post{p_1} \neq \post{p_2}$). If $|\bigcap_{p \in P'}\pre{p}| > 1 \ \vee \  |\bigcap_{p \in P'}\post{p}| > 0$, then a new place $p_{new}$ and a new silent transition $t_{new}$ are introduced. The shared incoming and outgoing arcs from/to $P'$ are redirected to $p_{new}$, $p_{new}$ is connected to $t_{new}$, and $t_{new}$ is connected to all places in $P'$. This transformation is illustrated in \autoref{fig:preprocessing:b}.
    
%     \item \textbf{Identical Post-Sets and Different Pre-Sets:} Let $P' \subseteq P$ a set of places of maximum size such that the places share the exact same post-set but have different pre-sets (i.e., $\forall_{p_1, p_2 \in P'}\ \post{p_1} = \post{p_2} \ \wedge \ \exists_{p_1, p_2 \in P'}\ \pre{p_1} \neq \pre{p_2}$). If $|\bigcap_{p \in P'}\pre{p}| > 0 \ \vee \  |\bigcap_{p \in P'}\post{p}| > 1$, then a new place $p_{new}$ and a new silent transition $t_{new}$ are introduced. The shared incoming and outgoing arcs from/to $P'$ are redirected to $p_{new}$, $t_{new}$ is connected to $p_{new}$, and all places in $P'$ are connected to $t_{new}$. This transformation is illustrated in \autoref{fig:preprocessing:c}.
% \end{enumerate}
% \end{definition}


\begin{definition}[Normalization of Start Place]
Let $N = (P, T, F)$ be a Petri net and $p_s 
\in P$ be its start place. We define  
\[
\normalizestart{(N, p_s)} = 
\begin{cases}
    (P, T, F) & \text{if } \pre{p_s} = \emptyset, \\
    (P', T', F') & \text{otherwise}.
\end{cases}
\]
with $(P', T', F')$ constructed as follows:

\begin{itemize}
    \item $T' = T \cup \{t_{source}\}$ where $t_{source} \notin T$ is a fresh transition with $\lab(t_{start}) = \tau$,
    \item $P' = P \cup \{p_{source}\}$ where $p_{source} \notin P$ is a fresh place,
    \item $F' = F \cup \{(p_{source}, t_{source}), (t_{source}, p_s)\}$.

\end{itemize}
\end{definition}

\begin{definition}[Normalization of End Place]
Let $N = (P, T, F)$ be a Petri net and $p_e \in P$ be its end place. We define 
\[
\normalizeend{(N, p_e)} = 
\begin{cases}
    (P, T, F) & \text{if } \post{p_e} = \emptyset, \\
    (P', T', F') & \text{otherwise}.
\end{cases}
\]
with $(P', T', F')$ constructed as follows:

\begin{itemize}
    \item $T' = T \cup \{t_{sink}\}$ where $t_{sink} \notin T$ is a fresh transition with $\lab(t_{start}) = \tau$,
    \item $P' = P \cup \{p_{sink}\}$ where $p_{sink} \notin P$ is a fresh place,
    \item $F' = F \cup \{(p_e, t_{sink}), (t_{sink}, p_{sink})\}$.

\end{itemize}
\end{definition}

Let $N$ be a Petri net, $p_s \in P$ be its start place, and $p_e \in P$ be its end place. Then we define:
\[
\normalizeall{(N, p_s, p_e)} = \normalizeend{(\normalizestart{(N, p_s)}, p_e)}.
\]


